Approximation of corner polyhedra with families of intersection cuts

We study the problem of approximating the corner polyhedron using intersection cuts derived from families of lattice-free sets in $\mathbb{R}^n$. In particular, we look at the problem of characterizing families that approximate the corner polyhedron up to a constant factor, which depends only on $n$ and not the data or dimension of the corner polyhedron. The literature already contains several results in this direction. In this paper, we use the maximum number of facets of lattice-free sets in a family as a measure of its complexity and precisely characterize the level of complexity of a family required for constant factor approximations. As one of the main results, we show that, for each natural number $n$, a corner polyhedron with $n$ basic integer variables and an arbitrary number of continuous non-basic variables is approximated up to a constant factor by intersection cuts from lattice-free sets with at most $i$ facets if $i> 2^{n-1}$ and that no such approximation is possible if $i \leq 2^{n-1}$. When the approximation factor is allowed to depend on the denominator of the fractional vertex of the linear relaxation of the corner polyhedron, we show that the threshold is $i > n$ versus $i \leq n$. The tools introduced for proving such results are of independent interest for studying intersection cuts.

==> f_metric.tex <==
% !TEX root = approx_corner.tex
\section{The $f$-metric}\label{sec:f_metric}

We give an example highlighting the need for a metric and the topological assumption of $\cB$ closed when characterizing the finite-approximation conditions $\rho_f(\cB, \cL)<\infty$ and $\rho(\cB, \cL)<\infty$. 


\begin{example}
Let $L\subseteq \R^2$ be a maximal lattice-free split (see~\cite[page 196]{conforti2014integer}). Choose $f\in \intr(L)$ and let $\cB\subseteq \cL_3^2\cap\cC_f$ be the set of all maximal lattice-free triangles containing $f$ in the interior. Since $L$ is a split, there is a nonzero vector $r$ in the lineality space of $L$. The intersection cut $C_L(r,f)$ is empty while $C_{B}(r,f)$ is nonempty for each $B\in \cB$. Hence $\rho_f(B, L) = \infty$ for each $B\in \cB$. However, it was shown in~\cite{bbcm} that $\rho_f(\cB,L) \leq 1$. 
\end{example}

Note that valid inequalities from $L$ (that is, the inequalities defining $L$-cuts) can be obtained by taking a limit of valid inequalities from a sequence of sets in $\cB$, and in the example we have seen valid inequalities from $L$ that cannot be obtained directly using one set $B\in \cB$ rather than a sequence. This explains the need of an appropriate topology and the necessity of topological-closedness assumptions on the family $\cB$ in Theorem~\ref{thmFinitenessFamilyFamily}. We induce such a topology using a metric, called the $f$-metric, which relies on the Hausdorff metric and polar bodies. The Hausdorff metric $d_H$ is defined on the family of compact sets of $\R^n$ as follows: $d_H(A,B)$ for compact sets $A,B$ is the minimum $\epsilon>0$ such that $A \subseteq B + N(0, \epsilon)$ and $B \subseteq A + D(0, \epsilon)$, where $D(0, \epsilon)$ is the open ball of radius $\epsilon$ around the origin. For a set $B\subseteq \R^n$, the polar of $B$ is $B^\circ:= \{r\in \R^n: r\cdot x\leq 1,~\forall x\in B\}$. 


For $f\in \R^n\setminus \Z^n$, recall that $\cC_f$ is the collection all closed, full-dimensional, convex sets in $\R^n$ that contain $f$ in their interior (see Definition~\ref{def:cC_f}).  We define the \emph{$f$-metric} $d_f:\cC_f\times \cC_f\to \R_{\geq 0}$ on $\cC_f$ to be
\begin{equation}
\label{metric_defn}
d_f(B_1, B_2) := d_H\left((B_1-f)^\circ, (B_2-f)^\circ\right),
\end{equation}
where $B_1, B_2\in \cC_f$. Note that $d_f(\cdot, \cdot)$ is always finite. This follows since $f\in \intr(B)$ for each $B\in \cC_f$, and the polar of a convex set is bounded if and only if the set contains the origin in its interior. %Furthermore, the polar of a set $B$ is independent of the representation of $B$ and therefore the $f$-metric is well-defined. 

Convergence in the $f$-metric is equivalent to pointwise convergence of gauge functions, as seen in the following proposition. We use $B_t\farrow B$ to denote convergence in the $f$-metric and $C_t\harrow C$ to denote convergence in the Hausdorff metric.

\begin{proposition}\label{prop:f_met_prop}
Consider $f\in \R^n\setminus \Z^n$. Let $(B_t)_{t=1}^\infty$ be a sequence of sets in $\cC_f$ and $B$ a set in $\cC_f$. The following are equivalent:

\begin{itemize}
\item[](a) $\psi_{B_t-f}$ converges to $\psi_{B-f}$ pointwise, as $t\to\infty$,
\item[](b) $\psi_{B_t-f}$ converges to $\psi_{B-f}$ on the unit sphere, as $t\to\infty$,
\item[](c) $\psi_{B_t-f}$ converges to $\psi_{B-f}$ uniformly on the unit sphere, as $t\to\infty$,
\item[](d) $(B_t-f)^\circ\harrow (B-f)^\circ$,
\item[](e) $B_t \farrow B$.
\end{itemize}
\end{proposition}
\begin{proof}
 The equivalence of $(a)$ and $(b)$ follows from~\eqref{eq:gauge_pos_hom}. The equivalence of $(c)$ and $(d)$ follows from Lemma 1.8.14 in~\cite{rsconvex}. It is immediate that $(c)$ implies $(ii)$. The fact that $(a)$ implies $(c)$ is true due to convexity of support functions (see, for example, Theorem 10.8 in~\cite{rock}). The equivalence of $(d)$ and $(e)$ follows by definition.
\end{proof}

\subsection{Properties of the $f$-metric}\label{sec:properties-f-metric}

Here we collect some notes on the $f$-metric, many of which follow from the next result from~\cite{rsconvex}. %We will use $\cl_f(\cdot)$ to denote the closure of a set under the $f$-metric.


\begin{theorem}[Theorem 1.8.8 in~\cite{rsconvex}]
	\label{thm:haus_prop}
	Let $(K_t)_{t=1}^\infty$ be a sequence of nonempty, convex, compact sets in $\R^n$ and $K\subseteq \R^n$ be nonempty, convex, and compact. Then $K_t\harrow K$ if and only if the following two conditions hold:
\begin{enumerate}
\item[](a) each point $x\in K$ is a limit of points $(x_t)_{t=1}^\infty$, where $x_t\in K_t$ for $t\in \N$; 
\item[](b) the limit of any convergent sequence $(x_{t_j})_{j=1}^\infty$, where $x_{t_j}\in K_{t_j}$ for $j\in \N$, is contained in $K$.
\end{enumerate}
\end{theorem}

Since we are concerned with intersection cuts, which are derived from lattice-free sets, our interest in the $f$-metric will restrict to lattice-free sets. The following result implies that lattice-free sets form a closed subset under the $f$-metric, and so limits of lattice-free sets are also lattice-free. 

\begin{proposition}	
	\label{prop:f_metric_properties}
	Let $f\in \R^n\setminus \Z^n$. Consider a sequence $(B_t)_{t=1}^\infty$ with $B_t\in\cC_f$ for every $t\in \N$ and a set $B\in \cC_f$ such that $B_t\farrow B$. Then
	\begin{itemize}
	\item[](a) if $x\in B_t$ for each $t\in \N$, then $x\in B$;
	\item[](b) if $x\not\in \intr(B_t)$ for each $t\in \N$, then $x\not\in \intr(B)$. 
	\end{itemize}

\end{proposition}

\begin{proof}
To prove (a), note that $x\in B_t$ is equivalent to $\psi_{B_t-f}(x-f)\leq 1$, and $x\in B$ to $\psi_{B-f}(x-f)\leq 1$. The result then follows from Proposition~\ref{prop:f_met_prop}. 

To prove (b), note that $x\not\in \intr(B_t)$ is equivalent to $\psi_{B_t-f}(x-f)\geq 1$, and $x\not\in\intr( B)$ to $\psi_{B-f}(x-f)\geq 1$. The result then follows from Proposition~\ref{prop:f_met_prop}. 
\end{proof}

While intersection cuts are expressed in terms of gauge functions, the $f$-metric is defined on convex sets. The next result states that the $f$-metric acts nicely when transitioning from convergence of lattice-free sets to convergence of their gauge functions (and consequently, to intersection cuts). 

\begin{proposition} \label{propContGuage}
	Let $f\in \R^n\setminus \Z^n$ and $B\in \cC_f$. Consider a sequence $(B_t)_{t =1}^{\infty}$ with $B_t\in \cC_f$ for each $t\in \N$ such that $B_t\farrow B$. Then $\psi_{B_t-f}\to \psi_{B-f}$ pointwise.
\end{proposition}

For a given set $S\subseteq \R^n$, the {\em support function} $\sigma_S$ is defined as $\sigma_S(r) = \sup_{x\in S}r\cdot x$. Proposition~\ref{propContGuage} follows from the fact that the gauge function of a set containing the origin in its interior is equal to the support function of the polar (see~\cite[Theorem 1.7.6]{rsconvex}), and the fact that if a family of compact, convex sets converge to a limit in the Hausdorff topology, then their support functions converge pointwise to the support function of the limit (see~\cite[Theorem 1.8.11]{rsconvex}).


For a family $\cB$ of lattice-free sets and some $f\in \R^n\setminus \Z^n$, the subfamily $\cB_f$ need not be closed under $d_f$ (indeed, this is the case for the family in the previous example). In this situation, the collection $\cB_f$ is a strict subfamily of $\cl_f(\cB_f)$. However, the next result states that the $\cB_f$-closure $C_{\cB_f}(R,f)$ is precisely the $\cl_f(\cB_f)$-closure. Moreover, these agree with the $\cB$-closure. Since $B$-cuts are defined by inequalities whose coefficients involve the gauge function $\psi_{B-f}$ and one can pass to a limit in inequalities, Proposition~\ref{prop:closure_equality} follows directly from Proposition~\ref{propContGuage}. 

\begin{proposition}
	\label{prop:closure_equality}
	Let $\cB$ be a family lattice-free convex sets in $\R^n$. Then $
		%\label{eq:closure_equality}
		C_\cB(R,f) = C_{\cB_f}(R,f) = C_{\cl_f(\cB_f)}(R,f)$
		 for every $(R,f)$. 
\end{proposition}

%\begin{proof}
%
%Choose a $(R,f)$ pair with $R\in \R^{n\times k}$ and $f\in \R^n\setminus \Z^n$. The equality $C_\cB(R,f) = C_{\cB_f}(R,f)$ holds because $C_B(R,f) = \R^{k}_{\geq0}$ for each $B\in \cB$ with $f\not\in \intr(B)$. So we focus our attention on the second equality. 
%
%Since $\cB_f\subseteq \cl_f(\cB_f)$, it follows that $C_{\cl_f(\cB_f)}(R,f) \subseteq C_{\cB_f}(R,f)$. In order to show $C_{\cB_f}(R,f) \subseteq C_{\cl_f(\cB_f)}(R,f)$, we derive
%$C_{\cB_f}(R,f) \subseteq C_B(R,f)$ for every $B \in \cl_f(\cB_f)$. Consider a sequence $(B_t)_{t \in \N}$ of elements of $\cB_f$
%converging to $B$ in the $f$-metric. Consider an arbitrary $s \in C_{\cB_f}(R,f)$. For each $t
%\in \N$ we have $\sum_{i=1}^k \psi_{B_t-f}(r_i)s_i \ge 1$ since $B_t \in \cB_f$.
%In view of Proposition~\ref{propContGuage}, in the latter inequality we can pass to
%the limit as $t \rightarrow \infty$ obtaining $\sum_{i=1}^k
%\psi_{B-f}(r_i) \ge 1$. Thus, $s \in C_B(R,f)$.
%\qed\end{proof}


In order to employ Theorem~\ref{thmFinitenessFamilyFamily}, we need to determine $\cl_f(\cB_f)$ for a family of lattice-free sets $\cB$ in $\R^n$. For $f\in \R^n\setminus \Z^n$, the family $\cL_i^n\cap \cC_f$ is closed under $d_f$. Therefore we can apply Theorem~\ref{thmFinitenessFamilyFamily} when proving results about the relative strength of $i$-hedral closures. 

\begin{proposition}
	\label{prop:i_hedral_closed}
	Let $i\in \N$ and $f\in \R^n\setminus \Z^n$. Then $\cl_f(\cL_i^n\cap \cC_f) = \cL_i^n\cap \cC_f$.
\end{proposition} 

\begin{proof}
Let $(B_t)_{t=1}^\infty$ be a sequence in $\cL_i^n\cap \cC_f$ and $B\in \cC_f$ such that $B_t\farrow B$. For $t\in \N$, $B_t$ has at most $i$ facets, so $(B_t-f)^\circ$ has at most $i$ vertices. Thus we may write $(B_t-f)^\circ  =\conv(a_{1,t},.., a_{i,t})$ for $a_{j,t}\in \R^n$ for $j\in [i]$, where some of $a_{1,t},.., a_{i,t}$ may coincide. Since the sequence of $(B_t-f)^\circ$ is bounded, the sequences $(a_{j,t})_{t=1}^\infty$ with $j\in [i]$ are all bounded. Therefore, after possibly taking subsequences, we may assume that $(a_{j,t})_{t=1}^\infty$ converges to some $a_j\in \R^n$ as $t\to\infty$. It follows that $\conv(a_{1,t},.., a_{i,t})$ converges to $\conv(a_{1},.., a_{i})$ as $t\to\infty$. Hence $(B-f)^\circ = \conv(a_{1},.., a_{i})$, showing $B$ has is a polyhedron with at most $i$ facets. 

\end{proof}

One should note that the collection $(\cL_i^n\setminus \cL_{i-1}^n)\cap \cC_f$ of polyhedra with exactly $i$-facets is not closed under $d_f$. However, its closure under the $f$-metric is $\cL_i^n\cap \cC_f$.
\begin{proposition}\label{prop:exactly_i_closed}
Let $f\in \R^n\setminus \Z^n$. For $i\geq 2$, $\cl_f((\cL_i^n\setminus \cL_{i-1}^n)\cap \cC_f) = \cL_i^n\cap \cC_f$.
\end{proposition}

\begin{proof}

Proposition~\ref{prop:i_hedral_closed} implies the $(\subseteq)$ direction of the conclusion. It is left to show the $(\supseteq)$ inclusion. It is sufficient to show that for every $B\in \cL_i^n\cap \cC_f$, there is a sequence of lattice-free sets $(B_t)_{t=1}^\infty$ in $(\cL_i^n\setminus \cL_{i-1}^n)\cap \cC_f$ that converges to $B$ in the $f$-metric. Equivalently, we would like to find a sequence of lattice-free sets $(B_t)_{t=1}^\infty$ such that $(B_t-f)^\circ\harrow(B-f)^\circ$ and $(B_t-f)^\circ$ has exactly $i$ facets for every $t\in \N$. Such a sequence can be made by modifying $(B-f)^{\circ}$. Indeed, if $(B-f)^{\circ}$ has $m\leq i$ vertices, then adding $i-m$ vertices outside and sufficiently close to $(B-f)^{\circ}$ yields $(B_t-f)^{\circ}$.

%We proceed with the following claim.
%
%\begin{Claim}\label{claim:at_most_i-1_facets}
%Let $j\geq 2$. Then $(\cL_{j-1}^n\setminus \cL_{j-2}^n)\cap \cC_f\subseteq  \cl_f((\cL_j^n\setminus \cL_{j-1}^n)\cap \cC_f)$.
%\end{Claim}
%
%\begin{cpf}
%Let $B\in (\cL_{j-1}^n\setminus \cL_{j-2}^n)\cap \cC_f$, and write $B$ as $B = \{x\in \R^n: a_j\cdot x\leq b_j, j\in [j-1]\}$. Consider a minimal face of $B$, defined by $B\cap \{x\in \R^n:c\cdot x= d\}$. For $t\in \N$, define $B_t:= B\cap \{x\in \R^n:c\cdot x \leq d-\frac{1}{t}\}$. Note that $B_t\subseteq B$ for every value of $t$, and therefore each $B_t$ is lattice-free. Also, since $f\in \intr(B)$, for large enough values of $t$ is follows that $f\in \intr(B_t)$. Finally, for large values of $t$, $B_t$ has exactly $j$ facets. Thus, for large values of $t$, $B_t\in (\cL_j^n\setminus \cL_{j-1}^n)\cap \cC_f$. Letting $t$ tend to infinity, it follows that $B_t\farrow B$, and so $B\in \cl_f((\cL_j^n\setminus \cL_{j-1}^n)\cap \cC_f)$ which proves the desired inclusion.
%
%\end{cpf}
%
%Let $j\leq i-1$. Using Claim~\ref{claim:at_most_i-1_facets} and the induction hypothesis, it follows that 
%$$(\cL_{j-1}^n\setminus \cL_{j-2}^n)\cap \cC_f\subseteq  \cl_f((\cL_j^n\setminus \cL_{j-1}^n)\cap \cC_f) = \cL_j^n\cap \cC_f\subseteq \cL_i^n\cap \cC_f.$$
%Also, using the fact that $ (\cL_i\setminus\cL_{i-1}^n)\cap \cC_f \subseteq \cl_f((\cL_i^n\setminus \cL_{i-1}^n)\cap \cC_f)$, we see that
%
%
%$$\cL_i^n\cap \cC_f = \bigcup_{j=2}^i (\cL_{j}^n\setminus \cL_{j-1}^n)\cap \cC_f\subseteq \cl_f((\cL_i^n\setminus \cL_{i-1}^n)\cap \cC_f),$$
%as desired. 

\end{proof}

Propositions~\ref{prop:closure_equality},~\ref{prop:i_hedral_closed}, and~\ref{prop:exactly_i_closed} support the examination of sets with at most $i$ facets instead of those with exactly $i$ facets. 

%The definition of an intersection cut is in terms of the gauge function of a lattice-free set, while the $f$-metric defined in Section~\ref{sec:f_metric} is on convex sets and not functions. 
















